Multi-Strided Access Patterns to Boost Hardware Prefetching

Important memory-bound kernels, such as linear algebra, convolutions, and stencils, rely on SIMD instructions as well as optimizations targeting improved vectorized data traversal and data re-use to attain satisfactory performance. On on temporary CPU architectures, the hardware prefetcher is of key importance for efficient utilization of the memory hierarchy. In this paper, we demonstrate that transforming a memory access pattern consisting of a single stride to one that concurrently accesses multiple strides, can boost the utilization of the hardware prefetcher, and in turn improves the performance of memory-bound kernels significantly. Using a set of micro-benchmarks, we establish that accessing memory in a multi-strided manner enables more cache lines to be concurrently brought into the cache, resulting in improved cache hit ratios and higher effective memory bandwidth without the introduction of costly software prefetch instructions. Subsequently, we show that multi-strided variants of a collection of six memory-bound dense compute kernels outperform state-of-the-art counterparts on three different micro-architectures. More specifically, for kernels among which Matrix Vector Multiplication, Convolution Stencil and kernels from PolyBench, we achieve significant speedups of up to 12.55x over Polly, 2.99x over MKL, 1.98x over OpenBLAS, 1.08x over Halide and 1.87x over OpenCV. The code transformation to take advantage of multi-strided memory access is a natural extension of the loop unroll and loop interchange techniques, allowing this method to be incorporated into compiler pipelines in the future.

==> texfiles/plots/comparison/cascade.tex <==
\begin{tikzpicture}
\begin{axis}[
    % x tick label style={rotate=14},
    ybar=0.05cm,
    legend style={at={(0.46,-0.2)},
      anchor=north,legend columns=-1},
    ylabel={Speedup},
    symbolic x coords={bicg,doitgen,gemver,mxv},
    xtick=data,
    ymin=0,
    ymax=6,
    visualization depends on={rawy \as \rawy},
    nodes near coords={\pgfmathtruncatemacro{\rawytrunc}{ifthenelse(\rawy==0,0,1)}\ifnum\rawytrunc=0\else\pgfmathprintnumber\rawy\fi},
    nodes near coords align={vertical},
    nodes near coords style={scale=0.6,rotate=90,anchor=west,fill=white},
    restrict y to domain*={\pgfkeysvalueof{/pgfplots/ymin}:\pgfkeysvalueof{/pgfplots/ymax}},
    enlarge x limits=0.006cm,
    bar width=0.33cm,
    height=4cm,
    width= 12.04cm,
    legend columns=-1,
    legend cell align=left,
    ylabel near ticks,
    transpose legend,
    title={Cascade Lake},
    title style={xshift=3cm},
    ]

\addplot[fill=red!60] coordinates {(bicg, 6.868982357037855) (doitgen, 5.152721305680266) (gemver, 4.360064863151796) (mxv, 3.7980314910222153)}; % Default
\addplot[fill=blue!60] coordinates {(bicg, 5.348313841877881) (doitgen, 1.378434541676287) (gemver, 3.2283748647318906) (mxv, 1.8404958917851348)}; % Polly
\addplot[fill=green!60] coordinates {(bicg, 1.9044492897419205) (doitgen, 0.9556684368506118) (gemver, 1.217120753447696) (mxv, 1.1341436144030557)}; % MKL
\addplot[fill=orange!60] coordinates {(bicg, 1.984578123792005) (doitgen, 1.0218194412375894) (gemver, 1.2476582725690561) (mxv, 1.2038140680572211)}; % OpenBLAS
\addplot[fill=purple!60] coordinates {(bicg, 2.2630794373542846) (doitgen, 2.3544766143062823) (gemver, 1.3361110392288453) (mxv, 1.0040447265539858)}; % No-unroll
\addplot[fill=cyan!60] coordinates {(bicg, 1.039919563619193) (doitgen, 2.1798981815724416) (gemver, 1.3140383783242542)  (mxv, 1.0)}; % Single-stride


% \legend{Default, Polly, MKL, OpenBLAS, No-unroll, Single-stride}
\end{axis}

\begin{axis}[
    % x tick label style={rotate=14},
    ybar=0.05cm,
    % legend style={at={(0.46,-0.2)},
      % anchor=north,legend columns=-1},
    % ylabel={Speedup},
    symbolic x coords={conv,jacobi2d},
    xtick=data,
    ymin=0,
    ymax=6,
    visualization depends on={rawy \as \rawy},
    nodes near coords={\pgfmathtruncatemacro{\rawytrunc}{ifthenelse(\rawy==0,0,1)}\ifnum\rawytrunc=0\else\pgfmathprintnumber\rawy\fi},
    nodes near coords align={vertical},
    nodes near coords style={scale=0.6,rotate=90,anchor=west,fill=white},
    restrict y to domain*={\pgfkeysvalueof{/pgfplots/ymin}:\pgfkeysvalueof{/pgfplots/ymax}},
    enlarge x limits=0.018cm,
    bar width=0.33cm,
    height=4cm,
    width= 8.35cm,
    legend columns=-1,
    legend cell align=left,
    ylabel near ticks,
    transpose legend,
    at={(10.6cm,0)},
    yticklabel={\empty},
    ]

\addplot[fill=red!60] coordinates {(conv, 1.2164835263429514) (jacobi2d, 0.9798199109526472)}; % Default
\addplot[fill=blue!60] coordinates {(conv, 1.2136323930780852) (jacobi2d, 2.2025327560016903)}; % Polly
\addplot[fill=green!50!black] coordinates {(conv, 1.947487624604314) (jacobi2d, 1.0648244161885325)}; % Halide Mullapudi
\addplot[fill=yellow!60] coordinates {(conv, 1.0119216146825971) (jacobi2d, 1.0767557561560814)}; % Halide Adams
\addplot[fill=brown!60] coordinates {(conv, 4.509930867002111) (jacobi2d, 2.1086683678890683)}; % Halide Li
\addplot[fill=teal!60] coordinates {(conv, 1.573911132844368) (jacobi2d, 0.0)}; % OpenCV
\addplot[fill=purple!60] coordinates {(conv, 1.260861735524674) (jacobi2d, 1.0491385984948787)}; % No-unroll
\addplot[fill=cyan!60] coordinates {(conv, 1.0046685340802988) (jacobi2d, 1.0226854691628062)}; % Single-stride


% \legend{Default, Polly, Halide Mullapudi, Halide Adams, Halide Li, OpenCV, No-unroll, Single-stride}
\end{axis}
\end{tikzpicture}

% \begin{verbatim}
    
% bicg
% {('duration_time', '4096'): [('mkl', 1.0806102613915416), ('polly', 0.38478808567306627), ('openblas', 1.0369798095238094), ('default', 0.2996029597726933)]}
% {('duration_time', 'bicgopt', '1073872896', '4096'): [(1, 1, 0.909365977537614), (16, 1, 1.9789679094339623), (20, 2, 2.0579674447949525)]}
% default 6.868982357037855
% polly 5.348313841877881
% mkl 1.9044492897419205
% openblas 1.984578123792005
% no_unroll 2.2630794373542846
% single_stride 1.039919563619193
% multi_stride 1.0
% {('duration_time', 'bicgopt', '1073872896', '4096'): [(1, 1, 1.8796750100744635), (3, 1, 1.9053523053435115), (3, 1, 1.9053523053435115)]}

% conv
% {('duration_time', '4096'): [('default', 1.640655075), ('halide', 0.4425411231359182), ('opencv', 1.2680702420228778), ('polly', 1.6445093938919342)]}
% {('duration_time', 'conv', '537002008', '4096'): [(1, 1, 1.5829093824613116), (9, 1, 1.9865555687732341), (18, 2, 1.9958298711484594)]}
% default 1.2164835263429514
% polly 1.2136323930780852
% halideMull 1.947487624604314
% halideAdams 1.0119216146825971
% halideLi 4.509930867002111
% opencv 1.573911132844368
% no_unroll 1.260861735524674
% single_stride 1.0046685340802988
% multi_stride 1.0

% doitgenliopt
% {('duration_time', '4096'): [('mkl', 0.010515606668277363), ('default', 0.001950315724650232), ('polly', 0.007290468341708543), ('openblas', 0.009834842616653485)]}
% {('duration_time', 'doitgenliopt', '72797760', '4096'): [(1, 1, 0.004268223912756695), (8, 1, 0.004610047144476935), (48, 8, 0.010049433387208496)]}
% default 5.152721305680266
% polly 1.378434541676287
% mkl 0.9556684368506118
% openblas 1.0218194412375894
% no_unroll 2.3544766143062823
% single_stride 2.1798981815724416
% multi_stride 1.0
% {('duration_time', 'doitgenliopt', '72797760', '4096'): [(1, 1, 0.009715759901237863), (1, 1, 0.009715759901237863), (13, 13, 0.009811326338253601)]}


% gemverliopt
% {('duration_time', '4096'): [('openblas', 0.5250008025037062), ('mkl', 0.5381730551333426), ('default', 0.1502320756475264), ('polly', 0.2028951474950665)]}
% {('duration_time', 'gemverliopt', '1074003968', '4096'): [(0, 0, 0.490244878694511), (1, 1, 0.4984798048170159), (2, 2, 0.6550215943491423)]}
% default 4.360064863151796
% polly 3.2283748647318906
% mkl 1.217120753447696
% openblas 1.2476582725690561
% no_unroll 1.3361110392288453
% single_stride 1.3140383783242542
% multi_stride 1.0

% jacobi2dopt
% {('duration_time', '4096'): [('halide', 0.10796565924844947), ('default', 0.2323526680062514), ('polly', 0.10336453333333333)]}
% {('duration_time', 'jacobi2dopt', '537001992', '4096'): [(1, 1, 0.2170006620689655), (34, 1, 0.22261367482014388), (34, 2, 0.22766377047549524)]}
% default 0.9798199109526472
% polly 2.2025327560016903
% halideMull 1.0648244161885325
% halideAdams 1.0767557561560814
% halideLi 2.1086683678890683
% opencv 0.0
% no_unroll 1.0491385984948787
% single_stride 1.0226854691628062
% multi_stride 1.0
% {('duration_time', 'jacobi2dopt', '537001992', '4096'): [(1, 1, 0.20862034772324067), (31, 1, 0.2159438692775152), (31, 1, 0.2159438692775152)]}

% mxvopt
% {('duration_time', '4096'): [('mkl', 2.145890996978852), ('openblas', 2.021698064516129), ('default', 0.6407920990601224), ('polly', 1.3223330637636082)]}
% {('duration_time', 'mxvopt', '1073807360', '4096'): [(1, 1, 2.4239443792325055), (3, 1, 2.4337485714285716), (3, 1, 2.4337485714285716)]}
% default 3.7980314910222153
% polly 1.8404958917851348
% mkl 1.1341436144030557
% openblas 1.2038140680572211
% no_unroll 1.0040447265539858
% single_stride 1.0
% multi_stride 1.0





% \end{verbatim}

==> texfiles/plots/comparison/coffee.tex <==
\begin{tikzpicture}
\begin{axis}[
    % x tick label style={rotate=14},
    ybar=0.05cm,
    legend style={at={(0.46,-0.2)},
      anchor=north,legend columns=-1},
    ylabel={Speedup},
    symbolic x coords={bicg,doitgen,gemver,mxv},
    xtick=data,
    ymin=0,
    ymax=6,
    visualization depends on={rawy \as \rawy},
    nodes near coords={\pgfmathtruncatemacro{\rawytrunc}{ifthenelse(\rawy==0,0,1)}\ifnum\rawytrunc=0\else\pgfmathprintnumber\rawy\fi},
    nodes near coords align={vertical},
    nodes near coords style={scale=0.6,rotate=90,anchor=west,fill=white},
    restrict y to domain*={\pgfkeysvalueof{/pgfplots/ymin}:\pgfkeysvalueof{/pgfplots/ymax}},
    enlarge x limits=0.006cm,
    bar width=0.33cm,
    height=4cm,
    width= 12.04cm,
    legend columns=-1,
    legend cell align=left,
    ylabel near ticks,
    transpose legend,
    title={Coffee Lake},
    title style={xshift=3cm},
    ]

\addplot[fill=red!60] coordinates {(bicg, 8.159172279451202) (doitgen, 12.06371565207844) (gemver, 5.286957788400138) (mxv, 4.388967281658275)};
\addplot[fill=blue!60] coordinates {(bicg, 4.162855600731059) (doitgen, 3.1862202597159492) (gemver, 3.196475180791706) (mxv, 2.2888758311707305)};
\addplot[fill=green!60] coordinates {(bicg, 1.140226744412832) (doitgen, 0.9822689998758397) (gemver, 1.1353588646354864) (mxv, 1.022276694999543)};
\addplot[fill=orange!60] coordinates {(bicg, 1.1254769731065157) (doitgen, 0.9972920057597395) (gemver, 1.1169385862545391) (mxv, 1.0404148246192075)};
\addplot[fill=purple!60] coordinates {(bicg, 1.426381013) (doitgen, 1.375134698) (gemver, 1.10011532502844) (mxv, 1.174469108585824)};
\addplot[fill=cyan!60] coordinates {(bicg, 1.411220516) (doitgen, 1.37518269) (gemver, 1.2365662599396658)  (mxv, 1.1663264021693176)};

% \legend{Default, Polly, MKL, OpenBLAS, No-unroll, Single-stride}
\end{axis}

\begin{axis}[
    % x tick label style={rotate=14},
    ybar=0.05cm,
    % legend style={at={(0.46,-0.2)},
      % anchor=north,legend columns=-1},
    % ylabel={Speedup},
    symbolic x coords={conv,jacobi2d},
    xtick=data,
    ymin=0,
    ymax=6,
    visualization depends on={rawy \as \rawy},
    nodes near coords={\pgfmathtruncatemacro{\rawytrunc}{ifthenelse(\rawy==0,0,1)}\ifnum\rawytrunc=0\else\pgfmathprintnumber\rawy\fi},
    nodes near coords align={vertical},
    nodes near coords style={scale=0.6,rotate=90,anchor=west,fill=white},
    restrict y to domain*={\pgfkeysvalueof{/pgfplots/ymin}:\pgfkeysvalueof{/pgfplots/ymax}},
    enlarge x limits=0.018cm,
    bar width=0.33cm,
    height=4cm,
    width= 8.35cm,
    legend columns=-1,
    legend cell align=left,
    ylabel near ticks,
    transpose legend,
    at={(10.6cm,0)},
    yticklabel={\empty},
    ]



\addplot[fill=red!60] coordinates {(conv, 1.5482441258406077) (jacobi2d, 1.0013883047036642)};
\addplot[fill=blue!60] coordinates {(conv, 1.5476350070341718) (jacobi2d, 1.6608964750927322)};
\addplot[fill=green!50!black] coordinates {(conv, 2.5349021811618715) (jacobi2d, 1.014034365302444)};
\addplot[fill=yellow!60] coordinates {(conv, 1.0825895543254969) (jacobi2d, 1.0143966759133363)};
\addplot[fill=brown!60] coordinates {(conv, 6.886211792056539) (jacobi2d, 3.5955536424328374)};
\addplot[fill=teal!60] coordinates {(conv, 1.8667635727776828) (jacobi2d, 0.0)};
\addplot[fill=purple!60] coordinates {(conv, 1.4247201035123356) (jacobi2d, 1.071167384)};
\addplot[fill=cyan!60] coordinates {(conv, 1.0584783928646873) (jacobi2d, 1.001345551)};

% \legend{Default, Polly, Halide Mullapudi, Halide Adams, Halide Li, OpenCV, No-unroll, Single-stride}
\end{axis}
\end{tikzpicture}


% \begin{verbatim}
% bicg
% default 8.159172279451202
% polly 4.162855600731059
% mkl 1.140226744412832
% openblas 1.1254769731065157
% no_unroll 1.426381013
% single_stride 1.411220516
% multi_stride 1.0
% (12, 6, 2.2257698398722883)
% (2, 1, 1.5771949279898312)
% (1, 1, 1.5604314829965622)

% conv
% default 1.5482441258406077
% polly 1.5476350070341718
% halideMul 2.5349021811618715
% halideAdams 1.0825895543254969
% halideLi 6.886211792056539
% opencv 1.8667635727776828
% no_unroll 1.4247201035123356
% single_stride 1.0584783928646873
% multi_stride 1.0

% doitgenli
% default 12.06371565207844
% polly 3.1862202597159492
% mkl 0.9822689998758397
% openblas 0.9972920057597395
% no_unroll 1.375134698
% single_stride 1.37518269
% multi_stride 1.0
% (33, 11, 0.021677809534497466)
% (1, 1, 0.015763585221075183)
% (1, 1, 0.0157641353706693)

% gemverliopt
% default 5.286957788400138
% polly 3.196475180791706
% mkl 1.1353588646354864
% openblas 1.1169385862545391
% no_unroll 1.10011532502844
% single_stride 1.2365662599396658
% multi_stride 1.0

% jacobi2dopt
% default 1.0013883047036642
% polly 1.6608964750927322
% halideMul 1.014034365302444
% halideAdams 1.0143966759133363
% halideLi 3.5955536424328374
% openCV 0.0
% no_unroll 1.071167384
% single_stride 1.001345551
% multi_stride 1.0
% (35, 5, 0.351325010304582)
% (4, 1, 0.350852919710816)
% (1, 1, 0.32798329706852675)

% mxvopt
% default 4.388967281658275
% polly 2.2888758311707305
% mkl 1.022276694999543
% openblas 1.0404148246192075
% no_unroll 1.174469108585824
% single_stride 1.1663264021693176
% multi_stride 1.0
% \end{verbatim}

==> texfiles/plots/comparison/legend.tex <==
\begin{tikzpicture}
\begin{axis}[
    legend style={at={(0.46,-0.2)},
      anchor=north,legend columns=-1},
    legend columns=-1,
    legend cell align=left,
    symbolic x coords={null},
    xtick=data,
    ybar=0.05cm,
    enlarge x limits=0.006cm,
    bar width=0.33cm,
    height=1pt,
    width=1pt,
]
%%%
\addplot[fill=red!60] coordinates {(null, 10)};
\addplot[fill=blue!60] coordinates {(null, 10)};
\addplot[fill=green!60] coordinates {(null, 10)};
\addplot[fill=orange!60] coordinates {(null, 10)};
\addplot[fill=green!50!black] coordinates {(null, 10)};
\addplot[fill=yellow!60] coordinates {(null, 10)};
\addplot[fill=brown!60] coordinates {(null, 10)};
\addplot[fill=teal!60] coordinates {(null, 10)};
\addplot[fill=purple!60] coordinates {(null, 10)};
\addplot[fill=cyan!60] coordinates {(null, 10)};
%%%
\legend{Default, Polly, MKL, OpenBLAS, Halide Mullapudi, Halide Adams, Halide Li, OpenCV, No-unroll, Single-stride}%%%
\end{axis}
\end{tikzpicture}


==> texfiles/plots/comparison/zen2.tex <==
\begin{tikzpicture}
\begin{axis}[
    % x tick label style={rotate=14},
    ybar=0.05cm,
    legend style={at={(0.46,-0.2)},
      anchor=north,legend columns=-1},
    ylabel={Speedup},
    symbolic x coords={bicg,doitgen,gemver,mxv},
    xtick=data,
    ymin=0,
    ymax=6,
    nodes near coords align={vertical},
    nodes near coords style={scale=0.6,rotate=90,anchor=west,fill=white},
    enlarge x limits=0.006cm,
    bar width=0.33cm,
    height=4cm,
    width= 12.04cm,
    legend columns=-1,
    legend cell align=left,
    ylabel near ticks,
    transpose legend,
    title={Zen 2},
    title style={xshift=3cm},
    visualization depends on={rawy \as \rawy},
    nodes near coords={\pgfmathtruncatemacro{\rawytrunc}{ifthenelse(\rawy==0,0,1)}\ifnum\rawytrunc=0\else\pgfmathprintnumber\rawy\fi},
    restrict y to domain*={\pgfkeysvalueof{/pgfplots/ymin}:\pgfkeysvalueof{/pgfplots/ymax}},
    % -----------------------------------------------------------------
    % we store the *original* y value in a variable ...
    % visualization depends on={rawy \as \rawy},
    % ... which value should be shown in the `nodes near coords' ...
    % nodes near coords={\pgfmathprintnumber\rawy},
    % ... and we want to limit the range of the bars to the axis limits
    % restrict y to domain*={
    %     \pgfkeysvalueof{/pgfplots/ymin}:\pgfkeysvalueof{/pgfplots/ymax}
    % },
    % -----------------------------------------------------------------
    ]

\addplot[fill=red!60] coordinates {(bicg, 18.756764175825037) (doitgen, 13.935342792609628) (gemver, 4.226056093531541) (mxv, 7.500482207542755)}; % Default
\addplot[fill=blue!60] coordinates {(bicg, 12.551053642847078) (doitgen, 3.6511343839886172) (gemver, 4.519418879804194) (mxv, 5.429741726431201)}; % Polly
\addplot[fill=green!60] coordinates {(bicg, 2.9911940906890226) (doitgen, 2.7033309006368476) (gemver, 2.3947183561928918) (mxv, 1.5558154973576872)}; % MKL
\addplot[fill=orange!60] coordinates {(bicg, 1.6170785665054943) (doitgen, 1.0846447642474506) (gemver, 0.7320148997886619) (mxv, 1.043208477451961)}; % OpenBLAS
\addplot[fill=purple!60] coordinates {(bicg, 1.743675425) (doitgen, 1.591610653) (gemver, 1.3016955022013088) (mxv, 1.6218073341856858)}; % No-unroll
\addplot[fill=cyan!60] coordinates {(bicg, 1.409114592) (doitgen, 1.58708949) (gemver, 1.3318701587035087)  (mxv, 1.2514380777403256)}; % Single-stride


% \legend{Default, Polly, MKL, OpenBLAS, No-unroll, Single-stride}
\end{axis}

\begin{axis}[
    % x tick label style={rotate=14},
    ybar=0.05cm,
    % legend style={at={(0.46,-0.2)},
      % anchor=north,legend columns=-1},
    % ylabel={Speedup},
    symbolic x coords={conv,jacobi2d},
    xtick=data,
    ymin=0,
    ymax=6,
    nodes near coords align={vertical},
    nodes near coords style={scale=0.6,rotate=90,anchor=west,fill=white},
    enlarge x limits=0.018cm,
    bar width=0.33cm,
    height=4cm,
    width= 8.35cm,
    legend columns=-1,
    legend cell align=left,
    ylabel near ticks,
    transpose legend,
    at={(10.6cm,0)},
    yticklabel={\empty},
    visualization depends on={rawy \as \rawy},
    nodes near coords={\pgfmathtruncatemacro{\rawytrunc}{ifthenelse(\rawy==0,0,1)}\ifnum\rawytrunc=0\else\pgfmathprintnumber\rawy\fi},
    restrict y to domain*={\pgfkeysvalueof{/pgfplots/ymin}:\pgfkeysvalueof{/pgfplots/ymax}},
    ]

\addplot[fill=red!60] coordinates {(conv, 3.0207209035846594) (jacobi2d, 0.8826285953934979)}; % Default
\addplot[fill=blue!60] coordinates {(conv, 3.015547308335525) (jacobi2d, 1.5710358837211509)}; % Polly
\addplot[fill=green!50!black] coordinates {(conv, 1.3502296784955305) (jacobi2d, 0.6937441484660468)}; % Halide Mullapudi
\addplot[fill=yellow!60] coordinates {(conv, 0.788584779642816) (jacobi2d, 0.7282006580990086)}; % Halide Adams
\addplot[fill=brown!60] coordinates {(conv, 5.942024534591359) (jacobi2d, 5.184837165692436)}; % Halide Li
\addplot[fill=teal!60] coordinates {(conv, 1.120155076411447) (jacobi2d, 0.0)}; % OpenCV
\addplot[fill=purple!60] coordinates {(conv, 1.1207198747131246) (jacobi2d, 1.226219641)}; % No-unroll
\addplot[fill=cyan!60] coordinates {(conv, 1.021175614095289) (jacobi2d, 1.206221621)}; % Single-stride


% \legend{Default, Polly, Halide Mullapudi, Halide Adams, Halide Li, OpenCV, No-unroll, Single-stride}
\end{axis}
\end{tikzpicture}


% \begin{verbatim}
% bicgopt
% default 18.756764175825037
% polly 12.551053642847078
% mkl 2.9911940906890226
% openblas 1.6170785665054943
% no_unroll 1.743675425
% single_stride 1.409114592
% multi_stride 1.0
% (10, 2, 3.882596253791844)
% (16, 1, 2.7553445809958816)
% (1, 1, 2.2266737246893182)


% conv
% {('duration_time', '4096'): [('opencv', 1.6647348957799792), ('halide', 1.3810696610261168), ('polly', 0.6183823544179471), ('default', 0.6173232496171134)]}
% {('duration_time', 'conv', '537002008', '4096'): [(1, 1, 1.6638959355160503), (12, 1, 1.8260926119346386), (10, 2, 1.864761244387225)]}
% default 3.0207209035846594
% polly 3.015547308335525
% halideMul 1.3502296784955305
% halideAdams 0.788584779642816
% halideLi 5.942024534591359
% opencv 1.120155076411447
% no_unroll 1.1207198747131246
% single_stride 1.021175614095289
% multi_stride 1.0

% doitgenliopt
% {('duration_time', '4096'): [('default', 0.001938757957730413), ('mkl', 0.009994062038986192), ('polly', 0.007399688395845498), ('openblas', 0.024908852763068666)]}
% {('duration_time', 'doitgenliopt', '106767360', '4096'): [(1, 1, 0.017121826151746202), (6, 1, 0.018791265903882547), (14, 7, 0.02701725673287307)]}
% default 13.935342792609628
% polly 3.6511343839886172
% mkl 2.7033309006368476
% openblas 1.0846447642474506
% no_unroll 1.591610653
% single_stride 1.58708949
% multi_stride 1.0
% (14, 7, 0.02701725673287307)
% (1, 1, 0.017023146399281375)
% (1, 1, 0.016974790084861684)

% gemverliopt
% {('duration_time', '4096'): [('mkl', 0.6010717805919278), ('polly', 0.3184917496373778), ('default', 0.3406006911683442), ('openblas', 1.966350175096983)]}
% {('duration_time', 'gemverliopt', '1074003968', '4096'): [(0, 0, 1.1057867404003914), (1, 1, 1.0807341969236688), (2, 2, 1.4393976263730357)]}
% default 4.226056093531541
% polly 4.519418879804194
% mkl 2.3947183561928918
% openblas 0.7320148997886619
% no_unroll 1.3016955022013088
% single_stride 1.3318701587035087
% multi_stride 1.0


% jacobi2dopt
% {('duration_time', '4096'): [('halide', 0.821900107104258), ('default', 0.6460116892915665), ('polly', 0.36293785255665173)]}
% {('duration_time', 'jacobi2dopt', '537001992', '4096'): [(1, 1, 0.5188775288804278), (14, 1, 0.5379003701589852), (22, 2, 0.5701883899271961)]}
% default 0.8826285953934979
% polly 1.5710358837211509
% halideMul 0.6937441484660468
% halideAdams 0.7282006580990086
% halideLi 5.184837165692436
% opencv 0.0
% no_unroll 1.226219641
% single_stride 1.206221621
% multi_stride 1.0
% (22, 2, 0.5701883899271961)
% (7, 1, 0.47270615950969813)
% (1, 1, 0.46499694743300385)

% mxvopt
% {('duration_time', '4096'): [('mkl', 2.4904842417140074), ('openblas', 3.714247020545507), ('polly', 0.7136129441152078), ('default', 0.5165979828986447)]}
% {('duration_time', 'mxvopt', '1073807360', '4096'): [(1, 1, 2.3891456756355565), (10, 1, 3.09622509343828), (42, 3, 3.8747339791837607)]}
% default 7.500482207542755
% polly 5.429741726431201
% mkl 1.5558154973576872
% openblas 1.043208477451961
% no_unroll 1.6218073341856858
% single_stride 1.2514380777403256
% multi_stride 1.0


% \end{verbatim}

==> texfiles/plots/rwc/copy.tex <==
\begin{tikzpicture}
  \begin{axis}[
      % xlabel={Number of strides},
      % ylabel={Throughput (GiB/s)},
      legend style={at={(0.5,-0.3)}, anchor=north, legend columns=2,cells={anchor=west}},
      title={Copy with Hardware Prefetching},
      xmin=0,
      xmax=33,
      width=1.15\textwidth,
      % ymin=500000000,
      % ymax=1025000000,
      xtick={1, 2, 4, 8, 16, 32},
      xticklabel=\empty,
      ytick={5, 10, 15, 20, 25, 30},
      scaled y ticks=true,
      % title style={yshift=2mm},
      height=4cm,
  ]
    
    \addplot[
      color=teal,
      thick,
      mark=square*,
      solid,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklasa_505290271_hwpf.csv};
    % \addlegendentry{AL-AS HWPF};

    % \addplot[
    %   color=orange,
    %   thick,
    %   mark=square,
    %   solid,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/writebacklasa_505290271_nohwpf.csv};
    % \addlegendentry{AL-AS};

    \addplot[
      color=cyan,
      thick,
      mark=triangle*,
      dashed,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklasnt_505290271_hwpf.csv};
    % \addlegendentry{AL-NTS HWPF};

    % \addplot[
    %   color=green!50!black,
    %   thick,
    %   mark=triangle,
    %   dashed,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/writebacklasnt_505290271_nohwpf.csv};
    % \addlegendentry{AL-NTS};

    \addplot[
      color=magenta,
      thick,
      mark=*,
      dotted,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklntsa_505290271_hwpf.csv};
    % \addlegendentry{NTL-AS HWPF};

    % \addplot[
    %   color=blue,
    %   thick,
    %   mark=o,
    %   dotted,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/writebacklntsa_505290271_nohwpf.csv};
    % \addlegendentry{NTL-AS};

    \addplot[
      color=brown,
      thick,
      mark=diamond*,
      dashdotdotted,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklntsnt_505290271_hwpf.csv};
    % \addlegendentry{NTL-NTS HWPF};

    % \addplot[
    %   color=red,
    %   thick,
    %   mark=diamond,
    %   dashdotdotted,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/writebacklntsnt_505290271_nohwpf.csv};
    % \addlegendentry{NTL-NTS};

    % \addplot[
    %   thick,
    %   color=orange,
    %   dotted,
    % ] 
    % coordinates {(0, 19.37) (33, 19.37)};
    % \addlegendentry{MLC All Reads}
    \addplot[
      thick,
      color=brown,
      dashdotted,
    ] 
    coordinates {(0, 19.02) (33, 19.02)};
    % \addlegendentry{STREAM Copy}
    \addplot[
      thick,
      color=blue,
      dashdotted,
    ] 
    coordinates {(0, 28.00) (33, 28.00)};
    % \addlegendentry{MLC 1:1 R/W}
  \end{axis}
    \begin{axis}[
      xlabel={Number of stride unrolls},
      % ylabel={Throughput (GiB/s)},
      legend style={at={(0.5,-0.3)}, anchor=north, legend columns=2,cells={anchor=west}},
      title={Copy without Hardware Prefetching},
      xmin=0,
      xmax=33,
      width=1.15\textwidth,
      % ymin=500000000,
      % ymax=1025000000,
      xtick={1, 2, 4, 8, 16, 32},
      xticklabels={%
        {1\hspace{3pt}}, % Add spacing before the label 1
        {\hspace{3pt}2}, % Add spacing after the label 2
        4, 8, 16, 32},
      ytick={5, 10, 15, 20, 25, 30},
      scaled y ticks=true,
      height=4cm,
      at={(0,-3.5cm)},
      % title style={yshift=2mm},
  ]
    
    % \addplot[
    %   color=orange,
    %   thick,
    %   mark=square*,
    %   solid,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/writebacklasa_505290271_hwpf.csv};
    % \addlegendentry{AL-AS HWPF};

    \addplot[
      color=teal,
      thick,
      mark=square*,
      solid,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklasa_505290271_nohwpf.csv};
    % \addlegendentry{AL-AS};

    % \addplot[
    %   color=green!50!black,
    %   thick,
    %   mark=triangle*,
    %   dashed,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/writebacklasnt_505290271_hwpf.csv};
    % \addlegendentry{AL-NTS HWPF};

    \addplot[
      color=cyan,
      thick,
      mark=triangle*,
      dashed,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklasnt_505290271_nohwpf.csv};
    % \addlegendentry{AL-NTS};

    % \addplot[
    %   color=blue,
    %   thick,
    %   mark=*,
    %   dotted,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/writebacklntsa_505290271_hwpf.csv};
    % \addlegendentry{NTL-AS HWPF};

    \addplot[
      color=magenta,
      thick,
      mark=*,
      dotted,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklntsa_505290271_nohwpf.csv};
    % \addlegendentry{NTL-AS};

% \addplot[
%       color=red,
%       thick,
%       mark=diamond*,
%       dashdotdotted,
%       mark options={solid},
%     ] 
%     table[
%       x index=0,
%       y index=1,
%       col sep=comma
%     ] {data/analysis/writebacklntsnt_505290271_hwpf.csv};
%     \addlegendentry{NTL-NTS HWPF};

    \addplot[
      color=brown,
      thick,
      mark=diamond*,
      dashdotdotted,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklntsnt_505290271_nohwpf.csv};
    % \addlegendentry{NTL-NTS};

    % \addplot[
    %   thick,
    %   color=orange,
    %   dotted,
    % ] 
    % coordinates {(0, 19.37) (33, 19.37)};
    % \addlegendentry{MLC All Reads}
    % \addplot[
    %   thick,
    %   color=brown,
    %   dashdotted,
    % ] 
    % coordinates {(0, 17.64) (33, 17.64)};
    % \addlegendentry{STREAM Copy}
    % \addplot[
    %   thick,
    %   color=violet,
    %   dashdotted,
    % ] 
    % coordinates {(0, 28.00) (33, 28.00)};
    % \addlegendentry{MLC 1:1 R/W}
  \end{axis}
\end{tikzpicture}



==> texfiles/plots/rwc/legend.tex <==
% Aligned
% Unaligned
% Non-temporal interleaved
% Non-temporal grouped
% Aligned load/Aligned store
% Non-temporal load/Non-temporal store
% Aligned load/Aligned store
% Non-temporal load/Non-temporal store

% MLC All reads
% MLC 1:1 R:W
% STREAM Copy

\begin{tikzpicture}
    \begin{axis}[
      legend style={at={(0.5,-0.5cm)}, anchor=south, legend columns=3,cells={anchor=west}},
      width=1cm,
      height=1cm,
  ]


    \addplot[
      color=orange,
      thick,
      mark=square*,
      mark options={solid},
      solid,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/readmultireg_505290271_nohwpf.csv};
    \addlegendentry{Aligned};
    \addplot[
      color=teal,
      thick,
      mark=square*,
      solid,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklasa_505290271_nohwpf.csv};
    \addlegendentry{Aligned Load/Aligned Store};
    \addplot[
      thick,
      color=red,
      dashdotted,
    ] 
    coordinates {(0, 19.38) (33, 19.38)};
    \addlegendentry{MLC All Reads}
    
    \addplot[
      color=green!50!black,
      thick,
      mark=triangle*,
      mark options={solid},
      dashed,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/readmultiregu_505290275_nohwpf.csv};
    \addlegendentry{Unaligned};
    \addplot[
      color=cyan,
      thick,
      mark=triangle*,
      dashed,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklasnt_505290271_nohwpf.csv};
    \addlegendentry{Aligned Load/Non-Temporal Store};
    \addplot[
      thick,
      color=blue,
      dashdotted,
    ] coordinates {(0, 28.00) (33, 28.00)};
    \addlegendentry{MLC 1:1 R/W}
    
    \addplot[
      color=blue,
      thick,
      mark=*,
      mark options={solid},
      dotted,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/readmultiregnt_505290271_nohwpf.csv};
    \addlegendentry{Non-Temporal Interleaved};
    \addplot[
      color=magenta,
      thick,
      mark=*,
      dotted,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklntsa_505290271_nohwpf.csv};
    \addlegendentry{Non-Temporal Load/Aligned Store};
    \addplot[
      thick,
      color=brown,
      dashdotted,
    ] 
    coordinates {(0, 19.02) (33, 19.02)};
    \addlegendentry{STREAM Copy}
    
    \addplot[
      color=purple,
      thick,
      mark=pentagon*,
      dashed,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/initmultiregnt2_505290271_nohwpf.csv};
    \addlegendentry{Non-Temporal Grouped};
    \addplot[
      color=brown,
      thick,
      mark=diamond*,
      dashdotdotted,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/writebacklntsnt_505290271_nohwpf.csv};
    \addlegendentry{Non-Temporal Load/Non-Temporal Store};

\end{axis}
  
\end{tikzpicture}



==> texfiles/plots/rwc/read.tex <==
\begin{tikzpicture}
  \begin{axis}[
      % xlabel={Number of strides},
      ylabel={Throughput (GiB/s)},
      ylabel style={xshift=-2cm},
      % legend style={at={(0.5,-0.3)}, anchor=north, legend columns=2,cells={anchor=west}},
      title={Read with Hardware Prefetching},
      xmin=0,
      xmax=33,width=1.15\textwidth,
      height=4cm,
      % ymin=500000000,
      % ymax=1025000000,
xtick={1, 2, 4, 8, 16, 32},
      xticklabel=\empty,      
      scaled y ticks=true,
      % title style={yshift=2mm},
  ]
    
    \addplot[
      color=orange,
      thick,
      mark=square*,
      mark options={solid},
      solid,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/readmultireg_505290271_hwpf.csv};
    % \addlegendentry{A HWPF};

    % \addplot[
    %   color=orange,
    %   thick,
    %   mark=square,
    %   mark options={solid},
    %   solid,
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/readmultireg_505290271_nohwpf.csv};
    % \addlegendentry{A};

    \addplot[
      color=green!50!black,
      thick,
      mark=triangle*,
      mark options={solid},
      dashed,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/readmultiregu_505290275_hwpf.csv};
    % \addlegendentry{U HWPF};

    % \addplot[
    %   color=green!50!black,
    %   thick,
    %   mark=triangle,
    %   mark options={solid},
    %   dashed,
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/readmultiregu_505290275_nohwpf.csv};
    % \addlegendentry{U};

    \addplot[
      color=blue,
      thick,
      mark=*,
      mark options={solid},
      dotted,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/readmultiregnt_505290271_hwpf.csv};
    % \addlegendentry{NT HWPF};

    % \addplot[
    %   color=blue,
    %   thick,
    %   mark=o,
    %   mark options={solid},
    %   dotted,
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/readmultiregnt_505290271_nohwpf.csv};
    % \addlegendentry{NT};

    \addplot[
      thick,
      color=red,
      dashdotted,
    ] 
    coordinates {(0, 19.38) (33, 19.38)};
    % \addlegendentry{MLC All Reads}
    % \addplot[
    %   thick,
    %   color=blue,
    %   dotted,
    % ] 
    % coordinates {(0, 26.94) (33, 26.97)};
    % \addlegendentry{STREAM Copy}
    % \addplot[
    %   thick,
    %   color=red,
    %   dotted,
    % ] 
    % coordinates {(0, 28.51) (33, 28.51)};
    % \addlegendentry{MLC 1:1 R/W}
  \end{axis}
  
    \begin{axis}[
      xlabel={Number of stride unrolls},
      % ylabel={Throughput (GiB/s)},
      legend style={at={(0.5,-0.3)}, anchor=north, legend columns=2,cells={anchor=west}},
      title={Read without Hardware Prefetching},
      xmin=0,
      xmax=33,
      width=1.15\textwidth,
      height=4cm,
      % ymin=500000000,
      % ymax=1025000000,
      xtick={1, 2, 4, 8, 16, 32},
      xticklabels={%
        {1\hspace{3pt}}, % Add spacing before the label 1
        {\hspace{3pt}2}, % Add spacing after the label 2
        4, 8, 16, 32},
      scaled y ticks=true,
      at={(0,-3.5cm)},
      % title style={yshift=2mm},
  ]
    
    % \addplot[
    %   color=orange,
    %   thick,
    %   mark=square*,
    %   mark options={solid},
    %   solid,
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/readmultireg_505290271_hwpf.csv};
    % \addlegendentry{A HWPF};

    \addplot[
      color=orange,
      thick,
      mark=square*,
      mark options={solid},
      solid,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/readmultireg_505290271_nohwpf.csv};
    % \addlegendentry{Aligned};

    % \addplot[
    %   color=green!50!black,
    %   thick,
    %   mark=triangle*,
    %   mark options={solid},
    %   dashed,
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/readmultiregu_505290275_hwpf.csv};
    % \addlegendentry{U HWPF};

    \addplot[
      color=green!50!black,
      thick,
      mark=triangle*,
      mark options={solid},
      dashed,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/readmultiregu_505290275_nohwpf.csv};
    % \addlegendentry{Unaligned};

    % \addplot[
    %   color=blue,
    %   thick,
    %   mark=*,
    %   mark options={solid},
    %   dotted,
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/readmultiregnt_505290271_hwpf.csv};
    % \addlegendentry{NT HWPF};

    \addplot[
      color=blue,
      thick,
      mark=*,
      mark options={solid},
      dotted,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/readmultiregnt_505290271_nohwpf.csv};
    % \addlegendentry{Non-Temporal Interleaved};

    \addplot[
      thick,
      color=red,
      dashdotted,
    ] 
    coordinates {(0, 19.38) (33, 19.38)};
    % \addlegendentry{MLC All Reads}
\end{axis}
  
\end{tikzpicture}



==> texfiles/plots/rwc/write.tex <==
\begin{tikzpicture}
  \begin{axis}[
      % xlabel={Number of strides},
      % ylabel={Throughput (GiB/s)},
      legend style={at={(0.5,-0.3)}, anchor=north, legend columns=2,cells={anchor=west}},
      title={Write with Hardware Prefetching},
      xmin=0,
      xmax=33,
      width=1.15\textwidth,
      % ymin=500000000,
      % ymax=1025000000,
      xtick={1, 2, 4, 8, 16, 32},
      xticklabel=\empty,
      scaled y ticks=true,
      height=4cm,
      % xtick={},
      % xmajorticks=false,
      % title style={yshift=2mm},
  ]
    
    \addplot[
      color=orange,
      thick,
      mark=square*,
      mark options={solid},
      solid,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/initmultireg_505290271_hwpf.csv};
    % \addlegendentry{A HWPF};

    % \addplot[
    %   color=orange,
    %   thick,
    %   mark=square,
    %   solid,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/initmultireg_505290271_nohwpf.csv};
    % \addlegendentry{A};

    \addplot[
      color=green!50!black,
      thick,
      mark=triangle*,
      mark options={solid},
      dashed,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/initmultiregu_505290275_hwpf.csv};
    % \addlegendentry{U HWPF};

    % \addplot[
    %   color=green!50!black,
    %   thick,
    %   mark=triangle,
    %   dashed,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/initmultiregu_505290275_nohwpf.csv};
    % \addlegendentry{U};

    \addplot[
      color=blue,
      thick,
      mark=*,
      dotted,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/initmultiregnt_505290271_hwpf.csv};
    % \addlegendentry{NT HWPF};

    % \addplot[
    %   color=red,
    %   thick,
    %   mark=diamond,
    %   dashdotted,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/initmultiregnt_505290271_nohwpf.csv};
    % \addlegendentry{NT};

    \addplot[
      color=purple,
      thick,
      mark=pentagon*,
      dashed,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/initmultiregnt2_505290271_hwpf.csv};
    % \addlegendentry{NT* HWPF};

    % \addplot[
    %   color=violet,
    %   thick,
    %   mark=pentagon,
    %   densely dotted,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/initmultiregnt2_505290271_nohwpf.csv};
    % \addlegendentry{NT*};

    % \addplot[
    %   thick,
    %   color=orange,
    %   dotted,
    % ] 
    % coordinates {(0, 19.37) (33, 19.37)};
    % \addlegendentry{MLC All Reads}
    % \addplot[
    %   thick,
    %   color=blue,
    %   dotted,
    % ] 
    % coordinates {(0, 26.94) (33, 26.97)};
    % \addlegendentry{STREAM Copy}
    % \addplot[
    %   thick,
    %   color=red,
    %   dotted,
    % ] 
    % coordinates {(0, 28.51) (33, 28.51)};
    % \addlegendentry{MLC 1:1 R/W}
  \end{axis}
  \begin{axis}[
      xlabel={Number of stride unrolls},
      % ylabel={Throughput (GiB/s)},
      legend style={at={(0.5,-0.3)}, anchor=north, legend columns=2,cells={anchor=west}},
      title={Write without Hardware Prefetching},
      xmin=0,
      xmax=33,
      width=1.15\textwidth,
      height=4cm,
      % ymin=500000000,
      % ymax=1025000000,
      xtick={1, 2, 4, 8, 16, 32},
      xticklabels={%
        {1\hspace{3pt}}, % Add spacing before the label 1
        {\hspace{3pt}2}, % Add spacing after the label 2
        4, 8, 16, 32},
      scaled y ticks=true,
      at={(0,-3.5cm)},
      % title style={yshift=2mm},
  ]
    
    % \addplot[
    %   color=orange,
    %   thick,
    %   mark=square*,
    %   solid,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/initmultireg_505290271_hwpf.csv};
    % \addlegendentry{A HWPF};

    \addplot[
      color=orange,
      thick,
      mark=square*,
      mark options={solid},
      solid,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/initmultireg_505290271_nohwpf.csv};
    % \addlegendentry{A};

    % \addplot[
    %   color=green!50!black,
    %   thick,
    %   mark=triangle*,
    %   dashed,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/initmultiregu_505290275_hwpf.csv};
    % \addlegendentry{U HWPF};

    \addplot[
      color=green!50!black,
      thick,
      mark=triangle*,
      mark options={solid},
      dashed,
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/initmultiregu_505290275_nohwpf.csv};
    % \addlegendentry{U};

    % \addplot[
    %   color=blue,
    %   thick,
    %   mark=*,
    %   dotted,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/initmultiregnt_505290271_hwpf.csv};
    % \addlegendentry{NT HWPF};

    \addplot[
      color=blue,
      thick,
      mark=*,
      dotted,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/initmultiregnt_505290271_nohwpf.csv};
    % \addlegendentry{NT};

    % \addplot[
    %   color=cyan,
    %   thick,
    %   mark=star,
    %   dashdotdotted,
    %   mark options={solid},
    % ] 
    % table[
    %   x index=0,
    %   y index=1,
    %   col sep=comma
    % ] {data/analysis/initmultiregnt2_505290271_hwpf.csv};
    % \addlegendentry{NT* HWPF};

    \addplot[
      color=purple,
      thick,
      mark=pentagon*,
      dashed,
      mark options={solid},
    ] 
    table[
      x index=0,
      y index=1,
      col sep=comma
    ] {data/analysis/initmultiregnt2_505290271_nohwpf.csv};
    % \addlegendentry{NT*};

    % \addplot[
    %   thick,
    %   color=orange,
    %   dotted,
    % ] 
    % coordinates {(0, 19.37) (33, 19.37)};
    % \addlegendentry{MLC All Reads}
    % \addplot[
    %   thick,
    %   color=blue,
    %   dotted,
    % ] 
    % coordinates {(0, 26.94) (33, 26.97)};
    % \addlegendentry{STREAM Copy}
    % \addplot[
    %   thick,
    %   color=red,
    %   dotted,
    % ] 
    % coordinates {(0, 28.51) (33, 28.51)};
    % \addlegendentry{MLC 1:1 R/W}
  \end{axis}
\end{tikzpicture}


==> texfiles/sections/3b_experiments_long.tex <==
Given the observations from our results for the simple data movement micro-benchmarks from Section~\ref{sec:analysis}, we will now determine the effect of multi-striding in practice.
For memory-bound compute kernels, we expect performance improvements when they are transformed to take advantage of multi-striding.
In this section, we first characterize the performance of multi-striding on six compute kernels of which many configurations have been generated. Secondly, we compare the performance of the best of our generated compute kernels to that of state-of-the-art implementations.
We conducted these experiments on three different micro-architectures to highlight the fact that multi-striding can be commonly applied.
%% KRIS: ik vond deze zin te ingewikkeld
%We expect similar effects to emerge within the domain of memory-bound compute kernels.
%, where the effect may be more prominent in some than others, depending on how much of a bottleneck data transfer for each particular kernel poses.
%Apart from the experiments themselves, in this section we provide the experimental setup for them among a description of the kernels used.

\subsection{Surveyed Kernels}
We explore six memory-bound kernels that are outlined in Table~\ref{tab:sizes}. The kernels marked with an asterisk are taken from PolyBench~\cite{polybench}. The gemver kernel consists of four separate steps that will be considered individually. Additionally, \emph{init} and \emph{writeback} kernels are included because some kernels include an initialization or write back phase as shown in the table.

The access type column (AT) shows whether the generated kernel uses aligned (A) or unaligned (U) memory accesses. 
Unaligned accesses are used for both stencil computations, as they involve padding, which offsets strides by values that break 32-byte alignment required for aligned instructions.
The strides column describes the memory access pattern generated by a kernel in terms of the number of load (L), store (S) and load/store (L/S) strides, where $n$ is the number of \emph{stride unrolls}. The table shows that we indeed selected  kernels that generate diverse memory access patterns.
Whether loop interchange (LI) and loop blocking (LB) were applied during the transformation of the compute kernel to a multi-strided variant is shown as well.

% dit was dubbel --Rob
%Furthermore, we list several characteristics for each kernel, such as whether an initialization step is present (IN), %whether a write-back step is included which copies values from one location to another (WB), whether the core %computational kernel is embedded in a number of loops (LE) and whether loop interchange was applied during the %transformation of the compute kernel to a multi-strided variant (LI).


% \subsubsection{Multi-striding in isolated computations}
%% KRIS: het zou kunnen dat deze paragraaf nog eentje naar boven moet. Daar ben ik nog niet uit.
These kernels will be used in the experiments presented in Sections~\ref{sec:striding_in_practice} and~\ref{sec:comparison}.
In the first set of experiments, we are interested in learning how effective the application of multi-striding is for the essential computation performed by each compute kernel.
However, compute kernels typically consist of multiple separate steps which exhibit different memory access patterns. 
To test the effect of a particular multi-striding configuration without interference of the other steps, we split these separate steps into isolated kernels.
This is indicated in the table by the initialization (IN), writeback (WB) and Loop Embedment (LE) columns.
More specifically, for doitgen and jacobi2d the unnecessary outer loops were removed as well as the initialization and writeback steps in general.
Loads and stores from each unroll are performed in these kernels, even if redundant.
This is to ensure comparable loop bodies in terms of amount and type of instructions, regardless of the multi-striding configuration.
As we empirically assessed aligned and interleaved accesses showed higher throughput than non-temporal and grouped accesses in all kernels, we use the former in these loop bodies for both experiments.
For the second set of experiments, where we compare to the state-of-the-art, we reassemble the compute kernels using the best striding configuration found for each of the separate steps.
We use 32-bit immediate addressing and problem sizes between 2 - 4 GiB such that these are divisible by the respective step sizes and facilitate aligned data movement (except for conv and jacobi2d which perform unaligned operations).

% Dat roept meer vragen op dan het beantwoordt. Bv: waarom is die 32 bit limiet bv anders voor de gesplitste kernels dan voor de combinatie? Dan moet je dat eigenlijk ook weer uitleggen, etc. --Rob
%Due to the 32-bit limit on immediate addressing and configuration dependent dimensionality constraints, the amount of data processed per kernel is limited and may deviate for the isolated computations and comparison to state-of-the-art.
%Enforcing the constraints on the dimensions of data lead us to multiple different data input sizes for the compute kernels. These data sizes are listed in Table~\ref{tab:sizes} under Data size.
%The data dimensions have been chosen such that these are divisible by the respective step sizes and facilitate aligned data movement (except for conv and jacobi2d which perform unaligned operations).


% : matrix vector multiplication (mxv), a 3x3 2D convolution stencil (conv), and from PolyBench: BiCG Sub Kernel of BiCGStab Linear Solver (bicg), Multi-resolution analysis kernel (MADNESS) (doitgen), Vector Multiplication and Matrix Addition (gemver) and 2-D Jacobi stencil computation (jacobi2d).
% As we empirically assessed aligned and interleaved accesses showed higher throughput than non-temporal and grouped accesses in all kernels, we mainly use the former.
% The conv and jacobi2d kernels use unaligned accesses, as they involve padding in the input and output data, which offsets strides by values that break 32-byte alignment.

%% Kernels and their parts
% Kernels can have their core embedded in loop structures and may consist of multiple parts.
% For instance, the doitgen kernel has its computation embedded in two loops and jacobi2d in a single.
% Furthermore, bicg and doitgen make use of an intialization step and doitgen and jacobi2d both have a writeback component where values are copied from one part of the memory to another.

% These consist of the double rank-1 matrix update (gemverouter), a transpose matrix vector multiplication (gemvermxv1), a vector sum update (gemversum) and the second matrix vector multiplication (gemvermxv2).
% Loop interchange is applied to the appropriate individual parts in doitgen and the transpose matrix vector multiplication part of gemver to facilitate adjacent accesses among loop iterations.

%Kernels may consist of multiple separate steps which may be broken up into isolated kernels to test the effect of a single striding configuration without interference of other parts.
%For instance, some kernels initialize some data structure before calculation, these two steps can be separately tested by isolation into an initialization and a calculation kernel.
% The computational parts of the six kernels generate different access patterns with different numbers of load and store sequences when $n$ strides are being used:
% \begin{itemize}[wide,noitemsep,labelwidth=!,labelindent=0pt]
% \item bicg: $n + 2$ load, $1$ store and $1$ load/store sequences.
% \item conv: $n + 2$ load and $n$ store sequences.
% \item doitgen: $n + 1$ load and $1$ load/store sequences.
% \item gemver: 
%     \begin{itemize}[wide,noitemsep,labelwidth=!,labelindent=4pt]
%     \item gemverouter: $4$ load and $n$ load/store sequences.
%     \item gemvermxv1: $n + 1$ load and $1$ load/store sequences.
%     \item gemversum: $n$ load and $n$ store sequences.
%     \item gemvermxv2: $n + 1$ load and $1$ load/store sequences.
%     \end{itemize}
% \item jacobi2d: $n + 2$ load and $n$ store sequences.
% \item mxv: $n + 1$ load and $1$ load/store sequences.
% \end{itemize}

\begin{table*}[h!]
\centering
\caption{Overview of the six surveyed compute kernels used in our experimentation.}%%
\label{tab:sizes}%%
\footnotesize%%
\begin{tabular}{|l|l||c||l|l|l||c|c|c|c||l|c|c|}\hline
 \multicolumn{2}{|c|}{\textbf{Kernel}}& \textbf{AT}& \multicolumn{3}{|c|}{\textbf{Strides}} & \multicolumn{5}{|c|}{\textbf{Characteristics}}& \multicolumn{2}{|c|}{\textbf{Data size (GiB)}}\\\hline
\textbf{Name}&\textbf{Description}&&\textbf{L}& \textbf{S}&\textbf{L/S} & \textbf{IN}&\textbf{WB} &\textbf{LE} &\textbf{LI} &\textbf{LB}& \textbf{Isolated}& \textbf{Comparison}\\\hline \hline
bicg*&BiCG Sub Kernel of BiCGStab Linear Solver &A& $n+2$& $1$&$1$ & Y& & & && 4                                      & 4                                   \\ \hline
conv                   &3x3 2D Convolution Stencil &U& $n+2$& $n$& & & & & && 2& 2\\ \hline
doitgen*&Multi-resolution analysis kernel (MADNESS) &A& $n+1$& &1 & Y& Y&2 &Y && 4                                      & 0.4\\ \hline
gemver*&Vector Multiplication and Matrix Addition &A& & & & & & & && & 4                                   \\ \hline 
- gemverouter*&  Double Rank-1 Matrix Update& A& $4$& & $n$ & & & & && 4&4\\ \hline 
- gemvermxv1*&  Transpose Matrix Vector Multiplication& A& $n+1$& & $1$ & & & &Y && 4&4\\ \hline 
- gemversum*& Vector Sum Update& A& $n$& $n$&  & & & & &Y& 4&4\\ \hline 
- gemvermxv2*& Matrix Vector Multiplication& A& $n+1$& & $1$ & & & & && 4&4\\\hline
jacobi2d*&2D Jacobi Stencil &U& $n+2$& $n$& & & Y&1 & && 2& 2                                   \\ \hline
mxv&Matrix Vector Multiplication &A& $n+1$& &1 & & & & && 4                                      & 4                                   \\ \hline
init&Initialization    &A& & $n$& & & & & &Y& 2                                      & 2                                   \\ \hline
writeback&Writeback    &A& $n$& $n$& & & & & &Y& 2                                      & 2                                   \\ \hline
\end{tabular}
\end{table*}



\subsection{Experimental Setup}
We consider the following micro-architectures: Intel(R) Core(TM) i7-8700 (Coffee Lake), Intel(R) Xeon(R) Silver 4214R (Cascade Lake) and AMD EPYC 7282 (Zen 2). We use the default page size (4 KiB). 
Further specifications are given in Table~\ref{tab:specs}.
%, where, among other specifications, we report the memory bandwidth for a single channel along with the number of channels, and the total cache size available per core. 
For both Intel micro-architectures, L3 is shared among all cores, but not for Zen 2.
All caches have a cache line size of 64 bytes.
On all machines, we use LLVM, CLang and Polly version 20.0.0, Halide version 18.0.0, MKL version 2024.2, OpenBLAS version 0.3.28 and OpenCV version 4.10.0.
The implementation of our kernels use the AVX2 instruction set extension using single-precision floating points (8 values per register).
For each experiment, we collect the median over 5 measurements, each including 5 executions.
%We calculated the single-thread Fused Multiply Add (FMA) theoretical peak performance (in GFLOPs per second) for the AVX2 extension with single-precision floating points.
%The peak performance for addition is half the FMA GFLOP/s in all three cases.
At the very end of each compute kernel, we place an \texttt{mfence} instruction to ensure all loads and stores are performed before measurement is stopped.

\input{texfiles/table/specs}

\subsection{Characterization of Multi-Striding}
\label{sec:striding_in_practice}
\input{texfiles/plots/kernels}
% * Wat willen we weten?
%In this experiment we verify the observed speedups in throughput from Section~\ref{sec:analysis} carry over to code that computational executions.
%We hypothesize that multi-striding will result in improved memory throughput for memory-bound compute kernels, similar to the effect seen in our analysis.
% * Hoe meten we dat / stellen we dat vast?
To characterize the effectiveness of multi-striding, we explore the optimization space of multi-striding for the isolated computational steps of the described compute kernels.
To do so, we evenly distribute a given total number of unrolls (1 up to 50) over a number of stride unrolls and portion unrolls.
This results in a large number of configurations and for each configuration we generate an AVX2-executable using our methodology described in Section~\ref{sec:approach}.
Note that for each number of stride unrolls we have multiple data points, namely one for each portion unrolled configuration.
For instance, given 6 unrolls, we may have 1 stride with a length of 6 vectors processed every iteration, 2 strides with length 3, 3 strides with length 2 and 6 strides of length 1.
%Given 4 unrolls, we may have 1 stride with a length of 4, 2 strides with a length of 2 and 4 strides with a length of 1.
%This already gives us two data points for configurations with 1 and 2 strides.
Because each of the stride configurations will have different divisibility constraints on the dimensions of the data, we report throughput rather than time to compare kernels operating on data of different sizes.

% * Resultaat (verwijzing figuur)
In Figure~\ref{fig:kernels} we plot the throughput of the different (isolated) compute kernels as a function of the number of stride unrolls.
The green horizontal line shows our baseline: the best performing single-strided kernel that uses only loop unrolls in the contiguous data axis.
The horizontal line in red indicates the throughput of the kernel that uses no unrolls.
The data points in the figures are colored with a gradient, according to the \emph{total} number of unrolls.
For brevity, we have left out the figures corresponding to the two matrix-vector multiplication operations of gemver, as they are equivalent to the mxv and loop interchanged doitgen kernels.

% * Analyse & conclusie.
The upper left and upper right graph show the throughput for the configurations for the bicg kernel with and without hardware prefetching, respectively.
From these results, it immediately becomes apparent that increasing the number of strides has a positive effect when hardware prefetching is enabled and has no significant effect otherwise. Multi-strided kernels overcoming the single-strided baseline when hardware prefetching is disabled is attributed to reduced loop overhead because of unrolling. This reaffirms that multi-striding takes better advantage of the available hardware prefetchers.

For all other results, hardware prefetching was enabled. There is a consistent trend among the different compute kernels, where a number of stride unrolls between 1 and 10 provides the highest throughput, before declining as this number increases.
As the gradient indicates, the number of total strides does not have a significant effect on the throughput.
Outliers often exist at striding configurations where the number of strides is a multiple of eight, which can be explained from cache collisions, as we discussed in Section~\ref{sec:cache-collisions}.

All results positioned above the green line surpass the best single-strided baseline configuration, showing multi-striding has a beneficial effect over default loop unrolling in the contiguous data axis.
For reference, as indicated by the red line, not considering loop unrolling at all leaves even more gains in performance untapped.  
%% KRIS: wil je nu nog iets zeggen over die rode lijn?  Hieronder wat oude tekst hier geparkeerd.
%We compare to the best performing single-strided variant as a baseline, to determine whether stride unrolling is favorable over loop unrolling in the contiguous data axis.
The jacobi2d kernel forms an exception: the performance of the best multi-strided variants is equal to, but not better than the best single-strided configuration.
When contrasting this to the conv kernel, which uses a similar access pattern given $n$ number of stride unrolls, we suspect a dependency with the computation performed; jacobi2d uses mostly additions, whereas conv uses fused multiply add instructions.
Apart from this exception, these results demonstrate that properly chosen kernel variations using our proposed multi-striding technique significantly outperform the single-strided baselines.
We observe speedups from a factor 1.02x for gemversum to a factor 1.58x for mxv.
% bicg 1.41
% conv 1.06
% doitgen 1.05
% gemverouter 1.11
% gemversum 1.02
% mxv 1.58
% Our results show that multi-striding with an appropriate number of strides provides an advantage over single-strided configurations for memory-bound kernels in practice.

% To summarize, for all isolated parts of relevant memory-bound kernels we have found evidence in favor of multi-striding over single strided implementations. We will now recombine these isolated parts into complete kernels without redundant loads and stores and compare their performance to various state-of-the-art implementations.

\subsection{Comparison with the State-of-the-Art}
\label{sec:comparison}
\input{texfiles/plots/comparison}
% * Wat willen we weten?
Now that we have confirmed that multi-striding is able to leverage the hardware prefetcher to obtain significant speedups over single-strided configurations for various compute kernels, we will show that our multi-strided compute kernels in many cases outperform state-of-the-art reference kernels.

%% DONE: onderstaande goed in deze sectie incorporeren
% \subsubsection{Multi-striding in optimized kernels}
% In the comparison with state-of-the-art of Section~\ref{sec:comparison}, we configure the initialization, writeback  and the four individual parts of gemver with the best configurations we found in isolated optimized kernels for these respective steps, to restrict the parameter space.
% We have removed the redundant load and store operations in our own kernel, but no elaborate optimizations have been performed.
% In the jacobi2d kernel, some intermediate results are recomputed, optimizations to counter this are not a part of multi-striding and are therefore not realized.
% Due to optimizing out redundant loads and stores, more vector registers will contain live values during the actual computation, restricting the space of feasible striding configurations.

% leading to a reassessment of the optimal numbers of strides for all kernels.

% % * Hoe meten we dat / stellen we dat vast?
%% Our kernels
To reduce the parameter space of kernels consisting of multiple parts, we focus on optimizing each part individually by isolating their performance exploration.
For example, in the gemver kernel, we configure each of its four individual parts using the highest-performing configurations found in isolated tests, merging these to form a unified configuration. 
Similarly, we apply the best configurations for initialization and writeback.
%onderstaande zinnen kunnen wel weg, valt gewoon onder optimale configs kiezen... --Rob
%However, for doitgen, the writeback configuration was excluded from this strategy. 
%Combining the writeback configuration with that of the initialization and computation, it led to dimensions that could not be allocated nor computed within a reasonable amount of time.
%As this part of doitgen processed the least number of values, we chose to use a default non-unrolled configuration for it.
We have removed the redundant load and store operations in our generated compute kernels, but no elaborate optimizations have been performed.
For instance, in the jacobi2d kernel, some intermediate results are recomputed. Optimizations to counter this are not related to multi-striding and are therefore not considered.

%% Comparison specific
To compare fairly against the different implementations, we display the highest recorded throughput among the used sizes of the data, per benchmark and micro-architecture.
Each of our best performing multi-strided assembly implementations is compared to a default implementation optimized by the CLang compiler, an implementation that is optimized by the CLang compiler with Polly and its stripmine vectorizer enabled, a generated assembly without unrolling and the best performing single-strided assembly implementation.
Furthermore, the bicg, doitgen, gemver and mxv kernels we compare with Intel's MKL and OpenBLAS.
The conv and jacobi2d stencil computations are compared with Halide, which may use either of three auto-schedulers, Mullapudi~\cite{Mullapudi2016}, Adams~\cite{Adams2019} and Li~\cite{Li2018}.
The throughput of the conv kernel is also compared against OpenCV.
For all setups we have verified whether the state-of-the-art implementations make use of the AVX2 extension.
Consistently among machines, this was only not the case for the bicg and mxv kernels for Polly and the mxv kernel for the default CLang compiled baselines.
If a state-of-the-art implementation outperforms the corresponding best performing single-strided counterpart, but in turn is surpassed by our best multi-strided implementation, we have direct evidence that multi-striding is valuable.
 
% * Resultaat (verwijzing figuur)


In Figure~\ref{fig:comparison} we find the speedup of multi-striding over different state-of-the-art implementations. %for the six described compute kernels, along with the results for the non-unrolled and best single-strided %implementations.
Overall, our results show that our multi-strided kernels outperform most state-of-the-art references.

For Coffee Lake we consistently outperform most kernels, surpassing Halide for all autoschedulers.
For the kernels bicg, doitgen, gemver, mxv, conv, some state-of-the-art kernels perform better than our best single-strided implementation, while being surpassed by our multi-strided variant.
This shows that it indeed is multi-striding (and not loop-unrolling and hand written assembly) that increases performance beyond the state-of-the-art implementations.
%We are on par with the implementation using Intel's MKL for doitgen, but we did not improve over it.
Interestingly, the gemver kernel shows that when combining the optimal parts of the single-strided variants, there is a decrease in performance compared to the non-unrolled version.

%For Cascade Lake we also consistently outperform most alternatives.
%kernels, where multi-striding is used to overcome implementations of doitgen and gemver using OpenBLAS and both Intel MKL and OpenBLAS, respectively.
For Cascade Lake the best multi-strided mxv and jacobi2d implementations were as good as the single-strided implementations, which is explained by multiple different types of strides already appearing when having a single stride unroll.
We are on par with MKL on doitgen and the LLVM autovectorization in the default CLang compiler setting, because that version uses of shuffle and permutation instructions which we did not consider.%, but provide additional gains in terms of throughput.

%For Zen2 we also outperform most state-of-the-art implementations. Multi-striding for gemver and mxv resulted in surpassing OpenBLAS.
%Once more we see that the single-strided variant of gemver did not improve over the non-unrolled one, meaning that coalescing configured parts of kernels does not always lead to the best performance.
For Zen2 we also outperform most state-of-the-art implementations, but it is clear that the performance characteristics are quite different, especially compared with Halide. 

%but performed worse than OpenBLAS on gemver, Halide with the Adams autoscheduler on conv and the default optimized CLang variant among the Mullapudi and Adams autoschedulers on jacobi2d, while we consistently showed speedups over all three Halide schedulers on the other two micro-architectures.

% * Analyse & conclusie.
Summarizing, compute kernels generated using our multi-striding methodology achieve noteworthy speedups over state-of-the-art implementations on different micro-architectures, while only being slightly surpassed in a few cases.
Multi-striding was even able to surpass state-of-the-art (hand-optimized) kernels, such as Intel's MKL.
This shows that multi-striding provides obvious advantages over state-of-the-art implementations and also can be generically applied.
%Recombining multiple separate parts of a kernel does not always lead to optimal performance, as seen in the gemver kernel results, where the best single-strided configurations combined into a single implementation performs worse than the best non-unrolled variant.
%We found evidence where multi-striding improves over single-strided variants to directly surpass state-of-the-art implementations, some of which consisting of hand-optimized assembly, such as Intel MKL.
For the jacobi2d kernel in particular our multi-strided kernels did not always show speedups. 
We have analyzed this and found that this kernel could have been optimized further, however this requires an optimization that is currently not incorporated into our methodology. Yet, our multi-strided variant still presents a small speedup over the single-strided baseline.

%Our worst performing kernel in terms of speedups, jacobi2d, could have been optimized further, possibly making it better at exploiting the hardware prefetcher.
%However, as we mentioned earlier, this requires an optimization unrelated to multi-striding, common subexpression in this case, avoiding intermediate results to be recomputed.
%In summary, multi-striding is a generic method that adapts relevant memory-bound compute kernels with an obvious advantage over state-of-the-art implementations.


==> texfiles/table/sota.tex <==
\begin{table}[h]
    \centering
    \caption{Performance Metrics for Various Kernels}
    \begin{tabular}{|l|l|l|l|}
        \hline
        \textbf{Kernel}                        & \textbf{Type}         & \textbf{Duration Time (ns) DAS-6} & \textbf{Duration Time (ns) coffee lake} \\ \hline
        \multirow{12}{*}{\textbf{bicgopt}}     &                       & (1/1)                             & (1/1) \\
                                               & Striding              & 1887994400                        & 2150713089 \\
                                               & MKL                   & 3945500191                        & 2175927756 \\
                                               & OpenBLAS              & 2084060241                        & 2123930294 \\
                                               & Polly                 & 23787316180                       & 9753144460 \\ \cline{2-4}
                                               &                       & (4/1)                             & (12/1) \\
                                               & Striding              & 1848845885                        & 2151486708 \\
                                               & MKL                   & 3945500191                        & 2175803030 \\
                                               & OpenBLAS              & 2084060241                        & 2124413806 \\
                                               & Polly                 & 23787316180                       & 97528248 \\\cline{2-4}
                                               &                       & (4/2)                             & (12/6) \\
                                               & Striding              & 1243259618                        & 1368581779 \\
                                               & MKL                   & 3945500191                        & 2175803030 \\
                                               & OpenBLAS              & 2084060241                        & 2124413806 \\
                                               & Polly                 & 23787316180                       & 9752824800 \\ \hline
        \multirow{12}{*}{\textbf{conv}}        &                       & (1/1)                             & (1/1) \\
                                               & Striding              & 5263194762                        & 4032449110 \\
                                               & Halide                & 6424369748                        & 8638735141 \\
                                               & OpenCV                & 5328272927                        & 6107433302 \\
                                               & Polly                 & 14637752692                       & 6105305071 \\\cline{2-4}
                                               &                       & (15/1)                            & (21/1) \\
                                               & Striding              & 5070304373                        & 3737396371 \\
                                               & Halide                & 6424369748                        & 8540031923 \\
                                               & OpenCV                & 5328272927                        & 6019737357 \\
                                               & Polly                 & 14405631949                       & 5331802104 \\\cline{2-4}
                                               &                       & (15/3)                            & (21/3) \\
                                               & Striding              & 4609785824                        & 3148026396 \\
                                               & Halide                & 6522258820                        & 8540031923 \\
                                               & OpenCV                & 5397725639                        & 6019737357 \\
                                               & Polly                 & 14405631949                       & 5331802104 \\\hline
        \multirow{12}{*}{\textbf{doitgenliopt}}&                       & (1/1)                             & (1/1) \\
                                               & Striding              & 48271722799                       & 52161974875\\
                                               & MKL                   & 88628573767                       & 39324382509 \\
                                               & OpenBLAS              & 193175994916                      & 114067741069 \\
                                               & Polly                 & 338545290212                      & 124865883628 \\\cline{2-4}
                                               &                       & (18/1)                            & (21/1) \\
                                               & Striding              & nvt                               & nvt \\
                                               & MKL                   & nvt                               & nvt \\
                                               & OpenBLAS              & nvt                               & nvt \\
                                               & Polly                 & nvt                               & nvt \\\cline{2-4}
                                               &                       & (18/9)                            & (21/7) \\
                                               & Striding              & 26512388083                       & 10916422110\\
                                               & MKL                   & 73142031607                       & 10978845064 \\
                                               & OpenBLAS              & 163166216653                      & 33110579383 \\
                                               & Polly                 & 292687502325                      & 36250448300 \\\hline
        \multirow{12}{*}{\textbf{gemverliopt}} &                       &                                   & (1/1) \\
                                               & Striding              &                                   & 4549196356 \\
                                               & MKL                   &                                   & 5357694992 \\
                                               & OpenBLAS              &                                   & 5388320146 \\
                                               & Polly                 &                                   & 25360860204 \\\cline{2-4}
                                               &                       &                                   & (unroll) \\
                                               & Striding              &                                   & tba \\
                                               & MKL                   &                                   & tba \\
                                               & OpenBLAS              &                                   & tba \\
                                               & Polly                 &                                   & tba \\ \cline{2-4}
                                               &                       &                                   & (best) \\
                                               & Striding              &                                   & 1694810831 \\
                                               & MKL                   &                                   & 2005674522 \\
                                               & OpenBLAS              &                                   & 1992020207 \\
                                               & Polly                 &                                   & 5506223768 \\ \hline
        \multirow{9}{*}{\textbf{jacobi2dopt}}  &                       & (1/1)                             & (1/1) \\
                                               & Striding              & 4298132494                        & 6614155153 \\
                                               & Halide                & 4700536868                        & 6264744325 \\
                                               & Polly                 & 10212208424                       & 10670160502 \\\cline{2-4}
                                               &                       & (44/1)                            & (28/1) \\
                                               & Striding              & 4025997365                        & 5900114949 \\
                                               & Halide                & 4403621963                        & 5779023292 \\
                                               & Polly                 & 9569747509                        & 9788507550 \\\cline{2-4}
                                               &                       & (44/2)                            & (28/7) \\
                                               & Striding              & 3547812976                        & 5697471590 \\
                                               & Halide                & 4403621963                        & 5779023292 \\
                                               & Polly                 & 9569747509                        & 9788507550 \\\hline
        \multirow{12}{*}{\textbf{mxvopt}}      &                       & (1/1)                             & (1/1) \\
                                               & Striding              & 1840537685                        & 1558383596 \\
                                               & MKL                   & 2272408121                        & 1372212726 \\
                                               & OpenBLAS              & 1335603587                        & 1405077653 \\
                                               & Polly                 & 10462912994                       & 4599564899 \\\cline{2-4}
                                               &                       & (40/1)                            & (36/1) \\
                                               & Striding              & 1816709764                        & 1743312611 \\
                                               & MKL                   & 2057842483                        & 1246050663 \\
                                               & OpenBLAS              & 1273073119                        & 1268013101 \\
                                               & Polly                 & 14083233124                       & 3549933733 \\ \cline{2-4}
                                               &                       & (40/2)                            & (36/9) \\
                                               & Striding              & 1158659982                        & 1219071166 \\
                                               & MKL                   & 2057842483                        & 1246050663 \\
                                               & OpenBLAS              & 1273073119                        & 1268013101 \\
                                               & Polly                 & 14083233124                       & 3549933733 \\ \hline
    \end{tabular}
    \label{tab:performance_metrics}
    \caption{Duration time per kernel. The column \textbf{u/s} contains the amount of unrolls followed by the number of strides these are evenly distributed over. Due to the constraints on the dimensions of the data, we have run the state-of-the-art kernels for the same dimensions corresponding to the 1/1 single-strided and to the best u/s multi-strided kernels (that process the most data per second). Misschien ook nog u/1?}
\end{table}

